JAM: Controllable and Responsible Text Generation via Causal Reasoning and Latent Vector Manipulation

While large language models (LLMs) have made significant strides in generating coherent and contextually relevant text, they often function as opaque black boxes, trained on vast unlabeled datasets with statistical objectives, lacking an interpretable framework for responsible control. In this paper, we introduce JAM (Just A Move), a novel framework that interprets and controls text generation by integrating cause-effect analysis within the latent space of LLMs. Based on our observations, we uncover the inherent causality in LLM generation, which is critical for producing responsible and realistic outputs. Moreover, we explore latent vectors as fundamental components in LLM architectures, aiming to understand and manipulate them for more effective and efficient controllable text generation. We evaluate our framework using a range of tools, including the HHH criteria, toxicity reduction benchmarks, and GPT-4 alignment measures. Our results show that JAM achieves up to a 22% improvement over previous Controllable Text Generation (CTG) methods across multiple quantitative metrics and human-centric evaluations. Furthermore, JAM demonstrates greater computational efficiency compared to other CTG methods. These results highlight the effectiveness and efficiency of JAM for responsible and realistic text generation, paving the way for more interpretable and controllable models.

==> ARR_Oct2024/content/background.tex <==
\section{Background and Observations}
\label{sec:latent}
\subsection{Latent Space in LLMs}
\label{sec:gene}
Latent spaces have been investigated and used in many previous works on LLMs. The work \citet{bronziniunveiling} explores how factual knowledge is encoded into the latent space of different layers and utilizes this observation to facilitate tasks such as fact-checking and semantic understanding. Latent vectors are also considered to represent the intentions for LLMs generation \cite{jiang2023latent}. All these previous works demonstrate the importance and potential of understanding and using latent vectors for the controllable generation of LLMs. However, none of the previous research has comprehensively explored the causality within latent spaces and its effects on LLM generation. To further investigate how latent vectors play a role during generation, we use hh-rlhf data from \citet{bai2022traininghelpfulharmlessassistant}, the honest dataset from \citet{lin2022truthfulqameasuringmodelsmimic} and conduct the following experiments:

\begin{figure}[t]
    \centering
    \includegraphics[width=0.5\textwidth]{figures/latent_space_diff_gene.pdf}
    \caption{The average differences among latent vectors of LLMs at each decoding step. Different colors represent different layers.}
    % \vspace{-10pt}
    \label{fig: gene}
\end{figure}

\begin{figure}[t]
        \centering
        \includegraphics[width=0.5\textwidth]{figures/latent_space_diff.pdf}
        \caption{The average differences among latent vectors of LLMs for each layer. Different colors represent different tasks. Harmless and helpful datasets are from hh-rlhf \cite{bai2022traininghelpfulharmlessassistant} and honest dataset from TruthfulQA \cite{lin2022truthfulqameasuringmodelsmimic}.}
        % \vspace{-10pt}
        \label{fig: layer}
\end{figure}

\begin{itemize}[topsep=0pt,parsep=4pt,itemsep=0pt,leftmargin=15pt]
    \item  \textbf{The evolution and pattern of latent vectors during generation.}
    To understand how latent vectors develop and enable LLMs to output answers corresponding to distinct prompts, it is necessary to investigate the differences between latent vectors along different decoding steps. We select $N$ prompts $\{p_1 ... p_N\}$ each with $K$ tokens and let LLMs generate $M$ tokens to each one. We save the latent vectors, marked as $h^m_{i|l}$, of the generated token at layer $l$ of decoding step $m$ for prompt $p_i$. Then, we calculate the differences among $\{h^m_{1|l}...h^m_{N|l}\}$ as negative cosine similarity: 
    \begin{equation}\label{eq: cos_sim}
    \small
        \mathbf{d}(h^m_{i|l}, h^m_{j|l}) = - \frac{h^m_{i|l} \cdot h^m_{j|l}}{\|h^m_{i|l}\| \|h^m_{j|l}\|}
    \end{equation}
    
    where $i,j \in [1,N], m \in [1, M], l \in [1,L]$. In this experiment, we set $N$ to 10 and $M$ to 30, and compute average $\mathbf{d}(h^m_{p_i|l}, h^m_{p_j|l})$ for each decoding layer over $N$ prompts. As illustrated in Figure \ref{fig: gene}, we observe that the latent vectors progressively diverge as the generation process advances, indicating that they become increasingly specific and representative at later decoding steps. 
    
    \item \textbf{The layer-wise behaviors of latent vectors.} 
    \label{sec:layer}
    It is also crucial to analyze layer-wise behaviors to gain deeper insights into LLM generation. From the previous experiments, we observe that the latent vector of the last token during generation $h^{K+M}_i$ is more expressive, and the latent vector of the last token in the prefilling process $h^K_i$ encapsulates previous tokens' information of the prompt according to attention mechanism. To simplify while preserving essential information for each prompt $p_i$, we extract the latent vectors from these two tokens for every layer $l$ and concatenate them to form a new latent vector $h_{p_i|l}$. 
    \begin{equation}
    \label{eq:latent}
        h_{p_i|l}=[h^K_{i|l}, h^{K+M}_{i|l}]
    \end{equation}

    We calculate $\mathbf{d}(h_{p_i|l}, h_{p_j|l})$ according to Eq. (\ref{eq: cos_sim}) for every layer $l$. The results in Figure \ref{fig: layer} demonstrate that the latent vectors become increasingly stable and representative in layers beyond $15^{th}$, conveying more specific information. This characteristic allows for more effective control over LLM generation, enabling more precise manipulation of the output.
    
\end{itemize}

\subsection{Causality in LLMs}
\label{sec:causality}
Causal reasoning has been proven to be effective for generative tasks in different areas \cite{bose2022controllable, geiger2022inducing, stolfo2022causal}, and it enables generative models to produce more realistic and reliable output. In this section, we aim to reveal the existence of causality in latent spaces of LLM generations and the importance of considering causality in CTG. There are two research questions we want to answer:
\begin{enumerate}
    \item \textbf{If each attribute in LLM generation is separable by a linear binary classifier.} Such separability would suggest that the underlying structure of the latent space is well-organized and distinct for different attributes, making it possible to detect and manipulate specific attributes with minimal complexity and high efficiency, facilitating attribute-based control over the generated content.
    \item \textbf{If we are able to identify causality existing in LLM generation.} Understanding these causal links is essential for controlling the generation process in a way that retains the natural flow of language and ensures that interventions (such as manipulating certain attributes) result in coherent and logically consistent text. This could lead to more reliable, ethical, and explainable content.
\end{enumerate}

\begin{table}[h]
    \centering
    \caption{Latent vectors SVM classifier test accuracy.}
    \label{table:svm}
    \begin{tabular}{lc}
        \toprule
        \textbf{Attributes} & \textbf{SVM Classifier Accuracy} \\ \midrule
        Honest & 0.80 \\ 
        Helpful & 0.72 \\ 
        Harmless & 0.71 \\ \bottomrule
    \end{tabular}
\end{table} 

\noindent \textbf{Classifier:} 
Binary classifiers that predict the likelihood of an attribute based on input text can be employed to shape the output distribution to align with the specified attribute \cite{sitdikov2022classifiersbetterexpertscontrollable, liang2024controlled, dekoninck2024controlledtextgenerationlanguage}. 
These classifiers can capture attributes that are not easily detectable in natural language. Unlike previous approaches that use text as input, we utilize latent vectors, aiming to explain attributes at a more fundamental level. Additionally, the linear model offers more interpretability compared to more complex models, providing further opportunities to understand and leverage the linear classifier effectively.

In our experiments, we train a classifier with decision boundary as hyperplane $S_A$ for latent vectors $h_{pi|l}$, as defined in Eq. (\ref{eq:latent}), for each attribute in the HHH criteria, using datasets with over 1000 data points for each and an 8:2 train-test split. Based on our observation in Figure \ref{sec:latent}, layers beyond the $15^{th}$ are more expressive. Thus, for all subsequent experiments, we set $l$ to $20^{th}$ layer, and simplify $h_{p_i|l}$ to $h_{p_i}$. The test accuracy results of Support Vector Machines (SVM) in Table \ref{table:svm} suggest that attribute patterns can be effectively captured in a linear manner.

\begin{table}[h]
    \centering
    \caption{Cause-effect correlation analysis with correlation coefficient ($\rho$) and $p$ value ($p$) on HHH criteria for both directions.}
    \label{table:causality}
    \begin{tabular}{llcc}
        \toprule
        \textbf{Cause} & \textbf{Effect} & \textbf{$\rho$} & \textbf{$p$} \\
        \midrule
        Honest & Harmless & 0.23 & 1.37e-024 \\ 
        Honest & Helpful & 0.66 & 2.50e-250 \\ 
        Harmless & Honest & 0.61 & 4.11e-149 \\ 
        Harmless & Helpful & 0.59 & 8.37e-140 \\ 
        Helpful & Honest & 0.63 & 1.20e-214 \\ 
        Helpful & Harmless & 0.24 & 9.34e-027 \\ \bottomrule
    \end{tabular}
\end{table}


\noindent \textbf{The existence of causality: } Consider a latent vector $h_{p_i}$, and a cause attribute $A_c$, where $A_c=1$ means this attribute exists in answers and 0 means it doesn't exist. 
\begin{align}
\label{eq:cf_mani}
    T_{A_c} &= h_{p_i} + \alpha S_{A_c} \\
    h_{p_i|A_c=1} &= T_{A_c}(h_{p_i|A_c=0} , \alpha)
\end{align}
$T_{A_c}$ is the latent vectors manipulation that we move the latent vector $h_{p_i}$ across the decision hyperplane by distance $\alpha$, in which the label for manipulated latent vector $h_{p_i|A_c=1}$ is calculated as $ S_{A_c} \cdot h_{p_i|A_c=1}=1$. The manipulation from $h_{p_i|A_c=1}$ to $h_{p_i|A_c=0}$ follows the same logic. 

Given latent vector $h_{p_i|A_c=0}$, we calculate its causality effect $\phi$ on a effect attribute $A_e$ as 
\begin{align}
\label{eq:effect}
    \phi = |S_{A_e} \cdot T_{A_c}(h_{p_i|A_c=0} , \alpha) - S_{A_e} \cdot h_{p_i|A_c=0}|
\end{align}
If $\phi=1$, it means the change of the label for cause attribute $A_c$ also causes the label for effect attribute $A_e$ to flip, $\phi=0$ otherwise. The similar logic is also followed by given input $h_{p_i|A_c=1}$. In Table \ref{table:causality}, we provide the causal effect estimates and their statistical significance for both directions. Here, all $p <= 0.05$ are typically considered statistically significant, and it indicates the confidence in the existence of a causal relationship.

It is important to explore and consider the causal relationships among attributes. When aiming to control a specific attribute, preserving the existing causality in LLMs is key to ensuring that the controlled text generation remains reliable and more aligned with natural language. We present a quantitative analysis of the effectiveness of this causal approach in Sec. \ref{sec:exp_gpt}, where the GPT-4 model demonstrates a preference for answers that account for causal relationships.

==> ARR_Oct2024/content/discussion.tex <==
\section{Conclusion}
In this paper, we proposed a novel framework, JAM, for responsible and controllable text generation. Our framework has demonstrated its strengths in controllable text generation by ensuring both reliability and realism through causality reasoning. It effectively enhances controllable text generation while providing deeper insights with high interpretability through latent vector manipulation. Additionally, JAM is versatile, capable of scaling across various attributes, and adapting to different LLMs. For future work, we are interested in exploring more complex manipulations involving specialized agent models. We are also interested in investigating how controllable text generation can be expanded beyond chatbots and question-answering systems to other applications.

%However, we acknowledge certain limitations in our method. When handling more complex requests, such as implicit preferences, the decision boundary may be insufficient in a single linear space. One potential approach to mitigate this issue is through the linear combination of decision boundaries, which requires further investigation. This includes exploring implicit attributes and developing more efficient and effective methods for latent space manipulation. Additionally, while JAM is computationally efficient, it sometimes requires LLMs to generate twice for effective latent space manipulation. Due to time and scope limitations, we have not addressed this issue in the current work, but we plan to tackle this limitation in future research.

\section{Limitations}
We acknowledge certain limitations of our method. When handling more complex requests, such as implicit preferences, the decision boundary may be insufficient in a single linear space. One potential approach to mitigate this issue is through the linear combination of decision boundaries, which requires further investigation. This includes exploring implicit attributes and developing more efficient and effective methods for latent space manipulation. Additionally, while JAM is computationally efficient, it sometimes requires LLMs to generate twice for effective latent space manipulation. Due to time and scope limitations, we have not addressed these issues in the current work, but we plan to tackle these limitations in the future.

\section{Acknowledgment}
We acknowledge the use of AI assistants based on GPT-4 to help us with the preparation of this manuscript.

==> ARR_Oct2024/content/experiments.tex <==
\begin{table*}
    \setlength\tabcolsep{4pt}
    % \vspace{-2mm}
    \centering
	\small
	\caption{Rouge2 and Bleurt scores on HHH-criteria tasks and perplexity of JAM with various hyper-parameters (marked as model\_name + $\alpha h$, i.e. \texttt{Llama3}$+ h$) compared with original \texttt{Meta-Llama-3-8B} and \texttt{Mistral-7B-Instruct-v0.2} models. Harmless and helpful datasets are from hh-rlhf \cite{bai2022traininghelpfulharmlessassistant} and honest dataset from TruthfulQA \cite{lin2022truthfulqameasuringmodelsmimic}. Scores are higher the better, perplexity is lower the better. We use bolded text to emphasize the model that achieves the best performance for each metric.}
	\label{table:hhh}
    % \vspace{-2mm}
	    \small
        \begin{tabular}{@{}
                l
                x{1}{3}
                x{2}{2}
                x{1}{3}
                x{2}{2}
                x{1}{3}
                x{2}{2}
                @{}
            }
            \toprule
            & \multicolumn{3}{c}{Harmless} & \multicolumn{3}{c}{Honest} & \multicolumn{3}{c}{Helpful} \\
            \cmidrule(lr){2-4}\cmidrule(lr){5-7}\cmidrule(lr){8-10}
             & \makecell{Rouge2}($\uparrow$) & {Bleurt}($\uparrow$) & {Perpl.}($\downarrow$) & \makecell{Rouge2}($\uparrow$)  & {Bleurt}($\uparrow$)  & {Perpl.}($\downarrow$)  & \makecell{Rouge2}($\uparrow$)   & {Bleurt}($\uparrow$)  & {Perpl.}($\downarrow$) \\
            \midrule
            $\texttt{Llama3}$ & 0.20 & 0.48 & 37.73 & 0.22 & 0.44 & \textbf{3.60} & 0.23 & 0.58 & \textbf{14.43}\\
            \texttt{Llama3}$+ h$ & \textbf{0.25} & \textbf{0.53} & 36.13 & \textbf{0.32} & \textbf{0.46} & 3.72 & \textbf{0.30} & 0.55 & 17.11\\
            \texttt{Llama3}$+ 1.2h$ & \textbf{0.25} & \textbf{0.53} & \textbf{36.10} & 0.29 & 0.44 & 3.80 & 0.25 & \textbf{0.65} & 19.70 \\
            \texttt{Llama3}$+ 1.5h$ & \textbf{0.25} & \textbf{0.53} & 36.25 & 0.30 & 0.45 & 4.00 & 0.25 & 0.60 & 23.80 \\
            \midrule
            $\texttt{Mistral}$ & 0.10 & 0.55 & \textbf{78.20} & 0.32 & 0.59 & 4.16 & 0.24 & 0.59 & 25.68 \\
            \texttt{Mistral}$+ h$ & \textbf{0.16} & 0.58 & 84.10 & \textbf{0.35} & \textbf{0.65} & \textbf{4.04} & \textbf{0.24} & \textbf{0.64} & 26.60\\
            % \texttt{Mistral}$+ 1.2h$ & \textbf{0.16} & 0.575 & 88.54 & \textbf{0.35} & 0.63 & 4.08 & 0.21 & 0.62 & \textbf{24.87} \\
            % \texttt{Mistral}$+ 1.5h$ & \textbf{0.16} & \textbf{0.585} & 88.50 & 0.31 & 0.61 & 4.36 & 0.19 & 0.60 & 29.19\\
            \texttt{Mistral}$+ 1.2h$ & \textbf{0.16} & 0.57 & 88.54 & \textbf{0.35} & 0.63 & 4.08 & 0.21 & 0.62 & \textbf{24.87} \\
            \texttt{Mistral}$+ 1.5h$ & \textbf{0.16} & \textbf{0.58} & 88.50 & 0.31 & 0.61 & 4.36 & 0.19 & 0.60 & 29.19\\
            \bottomrule
        \end{tabular}
\end{table*}

\begin{table*}[t]
    \centering
	\caption{Comparison of JAM with prompting method using GPT-4. GPT-4 is asked to choose the best response in terms of each task's requirement and relevance. Win/Lose/Draw indicates the percentage of times JAM wins, loses, or draws against the prompting method respectively. Here draw is the situation that GPT-4 chooses both.}
	\label{table:hhh_gpt4}
    % \vspace{-2mm}
        \begin{tabular}{lccc}
            \toprule
            & Harmless & Honest \\
            \cmidrule(lr){2-2}\cmidrule(lr){3-3}
            & Win / Lose / Draw & Win / Lose / Draw \\
            \midrule
            \texttt{Llama3}$ + h$ & \textbf{0.403} / 0.310 / 0.287 & \textbf{0.500} / 0.238 / 0.262 \\
            \texttt{Mistral}$ + h$ & \textbf{0.162} / 0.158 / 0.680 & \textbf{0.200} / \textbf{0.200} / 0.600 \\
            \bottomrule
        \end{tabular}
    % \vspace{-3mm}
\end{table*}

\begin{table*}
\centering
\caption{The average computation times for each stage of JAM using \texttt{Meta-Llama-3-8B}. JAM shows higher time efficiency compared with previous CTG work PREADD with the same setting and natural generation. Our method also shows negligible overhead for manipulation operations.}
\label{table:overhead}
\begin{tabular}{llcc}
\toprule
\textbf{Method} & \textbf{Process}& \textbf{Time (seconds)} & \textbf{Time Proportion} \\
\midrule
\multirow{4}{*}{JAM}
        & Latent Vectors Extraction &1.22 & 54.2\% \\
        \cmidrule(lr){2-4} 
        & Attribute Detection & 0.0006 & 0.03\% \\ \cmidrule(lr){2-4} 
        & Manipulation Vector Generation & 0.0005 & 0.02\% \\ \cmidrule(lr){2-4} 
        & Updated Generation & 1.03 & 45.76\%  \\ \midrule
PREADD & PREADD Generation & 6.51 & -- \\ \midrule
Original & Natural Generation & 1.22 & -- \\ \bottomrule
\end{tabular}
\label{tab:comparison}
\end{table*}

\section{Experiments}
\label{sec:exp}
To show that JAM is capable of scaling to and improving the score on different kinds of tasks, we evaluate our framework following HHH-criteria tasks. At the same time, we assess JAM with two popular LLMs: \texttt{Meta-Llama-3-8B} and \texttt{Mistral-7B-Instruct-v0.2} to demonstrate its feasibility with various kinds of LLMs. Furthermore, to better illustrate that JAM can help LLMs generate controllable and responsible answers that align with humans, we deploy GPT-4 as a human-like judge. 

\subsection{HHH Criteria}
We first assess JAM's effectiveness on tasks with different attributes. Using the HHH-criteria \cite{askell2021generallanguageassistantlaboratory} tasks, we show that JAM improves scores across all three criteria, evaluated using multiple metrics. The harmless and helpful datasets are sourced from hh-rlhf \cite{bai2022traininghelpfulharmlessassistant}, while the honest dataset is from TruthfulQA \cite{lin2022truthfulqameasuringmodelsmimic}. For each criterion, we train a binary classifier using 500 randomly selected data points. Labels for the training data are assigned by T5, assigning a label of 1 if the answer is closer to the correct example and vice versa. We then randomly draw 200 to 300 data points as a test set, ensuring no overlap with the training set to maintain fair evaluation. To thoroughly evaluate our model and align with widely-used metrics, we use BIG-bench \cite{srivastava2023beyond} as an evaluation tool. As shown in Table \ref{table:hhh}, JAM improves scores by up to 10\% and consistently outperforms the original models across all criteria.

We also demonstrate our method with different hyper-parameters $\alpha$ on both models. As expected, increasing $\alpha$ does not yield noticeable improvements. Since our classifier is binary and linear, moving further from the decision boundary does not necessarily reflect an absolute increase in any given attribute. Furthermore, while perplexity often indicates model confidence, it is not always a positive indicator if the model generates undesirable outputs. For example, in helpful criteria for \texttt{Mistral}$+h$ in helpful criteria, the score is improved by 7\%  even though the perplexity is not the lowest. 

\subsection{GPT-4 Preference}
\label{sec:exp_gpt}
It is also crucial to demonstrate that JAM enables LLMs to generate answers that are not only accurate but also relevant and fluent. To assess this, we compare our method with prompting techniques, which are widely used in CTG. We provide GPT-4 with two answers—one generated by JAM and the other using a prompting approach such as \textit{"You are a \{attribute\} assistant, please..."}. GPT-4 is then asked to choose one of the answers, both (draw), or neither. As shown in Table \ref{table:hhh_gpt4}, our method consistently outperforms the prompting approach across all three tasks, achieving a higher winning rate. This further highlights JAM’s ability to control LLMs to generate more coherent answers with desired attributes. For the helpful criterion, however, the ratio of “neither” responses exceeded any chosen answers, making it difficult to determine a clear winner, so we excluded this criterion from our discussion. This result may be related to the inherent capability of the original models in handling this attribute, which limits the potential improvement that could be achieved by the CTG method.

\subsection{Overhead Analysis}
We also aim to demonstrate the advantage of our method in terms of computational overhead. Due to the simplicity of our classifier, which is a binary and linear model, the training time is negligible. During inference, we record the average computation time for each stage of JAM using randomly selected inputs. Using \texttt{Meta-Llama-3-8B} as an example in Table \ref{table:overhead}, the computational load for generating the manipulation vector is nearly negligible, and the updated generation time is comparable to, or even faster than, the original natural generation. Furthermore, when comparing JAM to the previous CTG method, PREADD, our method demonstrates faster generation speed.

==> ARR_Oct2024/content/introduction.tex <==
\begin{figure*}[t]
        \centering
        \includegraphics[width=\textwidth]{figures/JAM_Flow.pdf}
        \caption{The framework of JAM. We first train a binary linear classifier regarding an attribute, such as harmless in scenarios. The details for classifier training are in Sec. \ref{sec:classifier}. During inference, it contains four steps: latent vector extraction, attribute detection, manipulation vector generation, and manipulate and update generation. The details for the inference are in Sec. \ref{sec:framework}.}
        \vspace{-10pt}
        \label{fig: jam_flow}
\end{figure*}

\section{Introduction}
Large Language Models (LLMs) have recently demonstrated remarkable capabilities across various domains, including question-answering, content creation, and reasoning. Chatbots, as one of the most popular interfaces for LLMs, engage diverse audiences—ranging from children to corporations—and these different user groups often prefer content with specific attributes. Given the expansive user base and various application scenarios, it is increasingly important to generate controllable content that aligns with desired attributes.

In Controllable Text Generation (CTG), one of the most common techniques for controlling LLMs is prompting \cite{NEURIPS2022_b1efde53}. While prompting is straightforward and easy to implement, it often falls short in steering LLMs in specific directions and producing reliable outputs consistently. Moreover, prompting lacks the ability to help people understand and interpret the generation process of LLMs, which is crucial for exerting precise control over their outputs. Another prevalent approach is fine-tuning LLMs; however, this method typically demands intensive computational resources and poses challenges in scaling up one fine-tuned model to accommodate the different desired attributes.

\noindent \textbf{Causal reasoning} offers a valuable framework for investigating and understanding the generative processes of LLMs \cite{xu2021causalitylearningnewperspective,leclair2021ensemblemodelsneuralsource, kaddour2022causalmachinelearningsurvey}. Traditional methods for controlling LLM outputs, such as prompting or fine-tuning, often treat the models as black boxes, making it difficult to predict or interpret their behaviors comprehensively. By contrast, causal reasoning enables us to model the internal mechanisms of LLMs more transparently, identifying how different components and latent variables influence the generated text. We believe that incorporating causality is essential for enhancing controlled text generation because it allows for systematic intervention in the generative process to achieve desired outcomes.

\noindent \textbf{Latent spaces in LLMs} are outputs of intermediate layers during computation, and serve as vital latent representations that encode the information and understanding LLMs utilize during text generation. These latent spaces convey various aspects of language, such as semantics, logics \cite{chen2024stateshiddenhiddenstates}, and hallucinations \cite{duan2024llms}, and are crucial for the model's ability to generate coherent and contextually appropriate responses. Therefore, by exploring and manipulating these latent vectors through the lens of causality, we see the potential to identify the cause-and-effect relationships that govern the model's behaviors. This approach should not only provide deeper insights into how LLMs process information but also establish a rigorous method to steer them toward generating reliable and desired responses.

In this paper, we investigate the causality inherent in popular LLMs and examine the consistency of inferred causal directions in Helpful, Honest, and Harmless (HHH) criteria tasks \cite{askell2021generallanguageassistantlaboratory}. Based on our observations of causal reasoning and latent vectors during generation, we propose a new framework, \textbf{JAM}~ (Just A Move) as shown in Figure \ref{fig: jam_flow}, that could control LLM generation by just a small move on latent vectors while preserving the original models' causality. JAM also ensures the quality and reliability of the generated outputs. For example, by intervening on specific latent states associated with undesirable attributes, we can suppress or modify these attributes in the output, thereby achieving more controlled and aligned text generation. Our contributions can be summarized as follows: 
\begin{enumerate}
    \item We investigate the behavior of latent vectors during LLM generation and uncover the existence of causal relationships within the latent spaces, specifically with respect to attributes in alignment tasks. We also provide statistical evidence for more insights. (Sec. \ref{sec:latent})
    \item Based on our observation, we propose the JAM framework shown in Figure \ref{fig: jam_flow}, which includes attribute classifier training and latent vectors manipulation to control LLM generation with negligible overhead. (Sec. \ref{sec:method})
    \item We conduct experiments of HHH-criteria on popular LLMs including Mistral-7B and Llama3-8B. JAM can improve up to 10\% scores on multiple metrics and win most of time on GPT-4 evaluation compared with traditional method. (Sec. \ref{sec:exp})
    \item We conduct ablation studies on the choices of parameters to provide more robust analysis and potential interpretations of the behaviors of LLMs' latent vectors. (Sec. \ref{sec:exp})
\end{enumerate}

==> ARR_Oct2024/content/method.tex <==
\begin{algorithm}
\caption{JAM Framework}
\begin{algorithmic}[1]
    \STATE \textbf{Input:} Dataset \{$p_1...p_N$\}, size $N$. LLM model $M$, attribute $A$.
    \STATE \textbf{Output:} Answers \{$a_1...a_N$\} with desired attributes.
    \FOR{$p_i$ in \{$p_1...p_N$\}}
        \STATE \textcolor{gray}{\textit{\# extract latent vectors}}
        \STATE $h^1_i ... h^{K+M}_i \gets M(p_i)$
        
        \STATE $h_{p_i} \gets [h^K_i, h^{K+M}_i]$
        \STATE \textcolor{gray}{\textit{\# detect attribute on attribute $A$}}
        \STATE $label \gets S_A \cdot h_{p_i}$
        \IF{$label == 0$}
            \STATE \textcolor{gray}{\textit{\# generate manipulation vector}}
            \STATE $\alpha \gets distance(h_{p_i},S_A)$
            \STATE \textcolor{gray}{\textit{\# manipulate and update generation}}
            \STATE Update $M(p_i)$ with  $\alpha S_A$
        \ENDIF \\
        $a_i = M(p_i)$
    \ENDFOR
    \STATE \textbf{Return} ${a_1...a_N}$
\end{algorithmic}
\end{algorithm}

\section{JAM Framework}
\label{sec:method}
With the observations summarized in Sec.~\ref{sec:latent}, we propose the JAM framework shown in Figure~\ref{fig: jam_flow} to train the attribute classifier and control the LLM output through latent vectors manipulation.

\subsection{Data Collection and Classifier Training}
\label{sec:classifier}
For the target LLMs, the dataset consists of prompts, LLM's answers, and the ground truth label given by the annotator regarding an attribute $A$. To automate the process in this project, instead of the given ground truth, we have a pair of correct answers and incorrect answers for each prompt. We use a text-to-text transfer transformer (T5) \cite{2020t5} to assign the label. It compares each generated answer with a correct and incorrect examples pair, assigning a label $y$ of 1 if the answer is closer to the correct examples and vice versa. After extracting latent vector $h_{p_i}$ described by Eq. (\ref{eq:latent}), we create dataset as \{$h_{p_i}, y_i$\}. The data is split into a training and testing set with an 8:2 ratio, totaling 500 data points, to train our binary classifier, as illustrated in the bottom left of Figure \ref{fig: jam_flow}. For classifier selection, we explore both SVM and logistic regression models, finding no significant difference in their performance.

\subsection{Latent Vector Manipulation During Inference} 

\label{sec:framework}
As shown in Figure~\ref{fig: jam_flow}, after classifier training, the JAM framework employs the classifier to manipulate latent vectors during inference. The manipulation process can be summarized into the following steps:
\begin{itemize}[topsep=0pt,parsep=4pt,itemsep=0pt,leftmargin=15pt]
    \item \textbf{Latent Vector Extraction:} we extract the representative latent vector for attribute detection and manipulation based on Eq. (\ref{eq:latent}). According to our observation in Sec. \ref{sec:latent}, this extracted vector conveys critical information for both the prefilling and generation stages, which aids the subsequent processes.
    \item \textbf{Attribute Detection:} during inference, given an input prompt and original answer, we first extract the latent vector $h_{p_i}$, and then let the trained classifier $S_A$ to decide if the answer contains the desired attribute $A$. If not, we move further to latent vector manipulation; otherwise, output the original answer.
    \item \textbf{Manipulation Vector Generation:} then we calculate the smallest distance $\alpha$ based on Eq.~(\ref{eq:cf_mani}) that could move $T_{A_c}(h_{p_i|A_c=0} , \alpha)$ to successfully generate vector $h_{p_i|A_c=1}$ with label 1. We use $\alpha S_A$ as a manipulation vector. 
    \item \textbf{Manipulate and Update Generation:} we update the latent vector of the last token of prefilling $h^K_{p_i}$ by adding the first half of the manipulation vector and gradually update the generated token by adding the second half of manipulation vector during each generation step.
\end{itemize}

==> ARR_Oct2024/content/related_work.tex <==
\section{Related Work}
 Several studies have explored CTG by adjusting a small fraction of the models' parameters during inference or using gradient-based methods. For example, \citet{yang2022unified} adjusts token distributions to ensure that toxic and biased attributes are not over-represented in the generated text, while \citet{dathathri2020plugplaylanguagemodels} uses Plug-and-Play Language Models (PPLM) to guide outputs via classifier gradients. However, both approaches are computationally expensive due to gradient updates or require extensive training data, limiting their scalability.

Alternative frameworks like DATG \cite{liang2024controlled} address CTG via dynamic attribute graphs to control keyword occurrences, but this method involves a time-consuming ranking process, especially for longer contexts, and the need to fine-tune embedding-based classifiers limits scalability across multiple attributes. Similarly, PREADD \cite{pei-etal-2023-preadd} modifies next-token probabilities by dividing the probabilities generated by a prefix with an undesired attribute from the original probabilities, generating new outputs. Fine-Grained Control via Model Arithmetic \cite{dekoninck2024controlledtextgenerationlanguage} takes a different approach by altering token probabilities through a linear combination of multiple LLMs prompted with different attributes, providing greater flexibility. However, this method is highly sensitive to prompt selection, which can reduce its reliability and scalability.

In summary, existing methods either have not effectively and efficiently addressed the challenges or introduced computational overhead. They fail to explain and control the generation process of LLMs at a fundamental level. 
